Past-present temporal programs over finite traces

Extensions of Answer Set Programming with language constructs from temporal logics, such as temporal equilibrium logic over finite traces (TELf), provide an expressive computational framework for modeling dynamic applications. In this paper, we study the so-called past-present syntactic subclass, which consists of a set of logic programming rules whose body references to the past and head to the present. Such restriction ensures that the past remains independent of the future, which is the case in most dynamic domains. We extend the definitions of completion and loop formulas to the case of past-present formulas, which allows capturing the temporal stable models of a set of past-present temporal programs by means of an LTLf expression.

==> include/asp-macros/automata.tex <==
% Automata
\newcommand{\AFA}{\ensuremath{\mathrm{AFA}}}
\newcommand{\automata}{\ensuremath{\mathfrak{A}}}
\newcommand{\run}{\ensuremath{G=(V,E)}}

% Word
\newcommand{\wT}{\ensuremath{w}}
 
% States
\newcommand{\q}[1]{\ensuremath{q_{#1}\,}}
\newcommand{\qstart}{\ensuremath{\q{{\textit{start}}}}}
\newcommand{\qleft}{\ensuremath{\q{\vdash}}}
\newcommand{\qright}{\ensuremath{\q{\dashv}}}

% Transition function
\newcommand{\fpbf}{\ensuremath{\bot}}
\newcommand{\tpbf}{\ensuremath{\top}}
\newcommand{\pbf}{\textit{pbf}}
% Transitions with sigma conditioned
\newcommand{\interp}{X}
\newcommand{\sigmaf}[1]{X_{#1}}
\newcommand{\sigmat}{\sigmaf{\top}}

\newcommand{\A}{\ensuremath{\mathcal{A }}}
\newcommand{\trace}{\T}

% 2AFA
\newcommand{\conf}[2]{\langle#1,#2\rangle}
\newcommand{\Tend}{\ensuremath{\vdash\T\dashv}}
\newcommand{\Tendl}{\ensuremath{\vdash \T_0 \cdots \T_{\lambda-1}\dashv}}

% Translations
\newcommand{\srtm}{\ensuremath{ST_m}}
\newcommand{\srtp}{\ensuremath{ST_p}}
\newcommand{\srtx}{\ensuremath{ST}}
\newcommand{\mso}{\text{mso}}


% ------ TIKZ 


% Rewrite Next to be able to import tikz 
\providecommand{\Next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\providecommand{\wNext}{\ensuremath{\widehat{\Next}}}

\usepackage{tikz} %Must go after macros
\usetikzlibrary{patterns,shapes.arrows,arrows,automata,positioning,trees,calc,shadows,positioning,fit,bending,fit}
\usepackage{tikz-cd}

\newcommand{\invisibleopac}{0.4}

\newcommand\addvmargin[1]{
  \node[fit=(current bounding box),inner ysep=#1,inner xsep=0]{};
}
\tikzset{
	arrows = {[bend]},
	>=latex',node distance=48pt,on grid,auto,initial text=,
	state/.style = {
		draw,
		circle,
		font=\footnotesize,
		minimum width=0.5cm,
		minimum height=0.5cm,
		fill=gray!10
	},
	config/.style = {
		font=\footnotesize
	},
	config_accept/.style = {
		config,
		color=green
	},
	trans/.style = {
		font=\tiny,
		color=gray
	},
	all/.style = {
		font=\scriptsize
	},
	run/.style = {
		-{Stealth[length=2.5, width=2.5]}
	},
	head/.style = {
		S-{Stealth[length=2.5, width=2.5]},
		sloped,
		inner sep = 0.6pt
	},
	headS/.style = {
		S-{Stealth[length=2.5, width=2.5]},
		sloped,
		inner sep = 0.6pt
	},
	headR/.style = {
		R-{Stealth[length=2.5, width=2.5]},
		sloped,
		inner sep = 0.6pt,
		color=blue
	},
	headL/.style = {
		L-{Stealth[length=2.5, width=2.5]},
		sloped,
		inner sep = 0.6pt,
		color=red
	},
	R/.tip = {%
		.[length=3]
		_[sep=2pt 2]
		Bar[sep=-1.7pt -2, length=0pt 1, width=3pt 3, line width=0.8]
		Bar[sep=1pt 0, length=3pt 3,width=0pt 1,line width=0.6]
	}, 
	every loop/.style={
		min distance=10mm,
		looseness=10
	},
	L/.tip = {%
		.
		_[sep=2pt 2]
		Bar[sep=1pt 0, length=3pt 3,width=0pt 1, line width=0.6]
	},
	S/.tip = {%
		.
	}
}


==> include/asp-macros/dtel.tex <==
\RequirePackage{bm}
\RequirePackage{textcomp}
\RequirePackage{upgreek}

\IfFileExists{outline.tex}{\input{outline}}{}

\newcommand{\next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\newcommand{\previous}{\text{\rm \raisebox{-.5pt}{\Large\textbullet}}}  % {{\ensuremath{\bullet}}}
\newcommand{\wnext}{\ensuremath{\widehat{\next}}}
\newcommand{\wprevious}{\ensuremath{\widehat{\previous}}}
\newcommand{\alwaysF}{\ensuremath{\square}}
\newcommand{\alwaysP}{\ensuremath{\blacksquare}}
\newcommand{\eventuallyF}{\ensuremath{\Diamond}}
\newcommand{\eventuallyP}{\ensuremath{\blacklozenge}}
\IfFileExists{outline.tex}
        {\newcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}}
        {\newcommand{\until}{\ensuremath{\mathbin{\bm{\mathsf{U}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}}
        {\newcommand{\release}{\ensuremath{\mathbin{\bm{\mathsf{R}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\while}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{W}}$}}}}}}
        {\newcommand{\while}{\ensuremath{\mathbin{\bm{\mathsf{W}}}}}}
\newcommand{\since}{\ensuremath{\mathbin{\bm{\mathsf{S}}}}}
\newcommand{\trigger}{\ensuremath{\mathbin{\bm{\mathsf{T}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}}
        {\newcommand{\finally}{\ensuremath{\bm{\mathsf{F}}}}}
\newcommand{\initially}{\ensuremath{\bm{\mathsf{I}}}}

\newcommand{\stp}{\ensuremath{\uptau}}
\mathchardef\mhyphen="2D
\newcommand{\prev}{\ensuremath{\stp^{\mhyphen}}}
\newcommand{\prevs}{\ensuremath{\stp^{\mhyphen *}}}

\newcommand{\dalways}[1]{\ensuremath{[#1]\,}}                        % \DBox
\newcommand{\DBox}[1]{\dalways{#1}}
\newcommand{\deventually}[1]{\ensuremath{\langle#1\rangle\,}}        % \DDia
\newcommand{\DDia}[1]{\deventually{#1}}
\newcommand{\drel}[2]{\ensuremath{{\parallel}{#1}{\parallel}^{#2}}}  % \Rel

\newcommand{\intervcc}[2]{\ensuremath{[#1..#2]}}
\newcommand{\intervco}[2]{\ensuremath{[#1..#2)}}
\newcommand{\intervoc}[2]{\ensuremath{(#1..#2]}}
\newcommand{\intervoo}[2]{\ensuremath{(#1..#2)}}
\newcommand{\rangecc}[3]{\ensuremath{#1 \in \intervcc{#2}{#3}}}
\newcommand{\rangeco}[3]{\ensuremath{#1 \in \intervco{#2}{#3}}}
\newcommand{\rangeoc}[3]{\ensuremath{#1 \in \intervoc{#2}{#3}}}
\newcommand{\rangeoo}[3]{\ensuremath{#1 \in \intervoo{#2}{#3}}}

\newcommand{\cl}[1]{\ensuremath{\mathit{cl}({#1})}}
\newcommand{\last}{\ensuremath{\mathit{last}}}


==> include/asp-macros/grounding.tex <==
\newcommand{\ground}[1]{\ensuremath{\mathit{ground}(#1)}}
\newcommand{\cground}[2]{\ensuremath{\mathit{ground}_{#2}(#1)}}

\newcommand{\vars}[1]{\mathit{vars}(#1)}
\newcommand{\match}[2]{\mathit{match}_{#2}(#1)}


==> include/asp-macros/listings.tex <==
% The language definitions below require the following packages:
%
%     \usepackage{courier}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%     \renewcommand{\Underscore}{\textscale{1}{\textunderscore}}
%
% Without extra packages I had to provide an alternative underscore definition
% to get decent looking underscores.
%
% As an alternative to courier, it is also possible to use the `lmodern`
% package.
%
%     \usepackage[T1]{fontenc}
%     \usepackage{lmodern}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%
% When the python or clingo language is given, tex code can be embedded
% escaping it in `#( ... #)`, which is treated like a comment in Python.
% Furthermore, for logic programs the character sequence is `%%` is not output.
% This can be used to add labels at the end of lines. For example, in a logic
% program one can write
%
%     H :- B.%%#( \label{lst:rule} #)
%
% to refer to the rule from the document without having to worry about changing
% line numbers when refactoring. The annotated program will still be runnable
% with clingo.

\providecommand{\Underscore}{\textunderscore}

\lstdefinelanguage{clingo}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  keywordstyle=[2]\bfseries,%
  keywordstyle=[3]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}1 {\%\%}{}0,%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  keywords=[2]{\#const,\#show,\#minimize,\#base,\#theory,\#count,\#external,\#program,\#script,\#end,\#heuristic,\#edge,\#project,\#show,\#sum},%
  keywords=[3]{&,&dom,&sum,&diff,&show},%
  morecomment=[l]{\#\ },%
  morecomment=[l]{\%\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}

\lstdefinelanguage{python}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}{1},%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  morecomment=[l]{\#\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}



==> include/asp-macros/modules.tex <==
% - modules ----------------------------------------
\newcommand{\module}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\prog}[1]{\ensuremath{P(#1)}}
\newcommand{\inp}[1]{\ensuremath{I(#1)}}
\newcommand{\out}[1]{\ensuremath{O(#1)}}
\newcommand{\inst}[2]{\ensuremath{#1(#2)}}
% \newcommand{\exts}{\epsilon}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> include/asp-macros/operators.tex <==

% - operators ------------------------------------------------------------------

\newcommand{\Top}[1]{\ensuremath{T_{#1}}}
\newcommand{\T}[2]{\Top{#1}#2}
\newcommand{\Topi}[2]{\Top{#2}^{#1}}
\newcommand{\Ti}[3]{\Topi{#1}{#2}#3}

% - semantic operators -----------------------------------------------------------

\newcommand{\SM}[1]{\ensuremath{\mathit{SM}(#1)}}


==> include/asp-macros/outline.tex <==
\RequirePackage{xcolor}
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/proof.tex <==
\newcounter{casenum}
\newenvironment{caseof}{\setcounter{casenum}{1}}{\vskip.5\baselineskip}
\renewenvironment{quote}{%
  \list{}{%
    \leftmargin15pt  
    \rightmargin0cm
  }
  \item\relax
}
{\endlist}


\newcommand{\case}[2]{\begin{quote} 
    \hspace{-10pt}{\bfseries \textit{Case} $\bm{#1}$}: #2\end{quote}\addtocounter{casenum}{1}}
\newcommand{\caselr}[1]{\begin{itemize}
    \item[\ensuremath{\bm{\Rightarrow)}}] #1\end{itemize}}
\newcommand{\caseeq}[1]{\begin{itemize}
    \item[\ensuremath{\bm{\Leftrightarrow )}}] #1\end{itemize}}
\newcommand{\caserl}[1]{\begin{itemize}
    \item[\ensuremath{\bm{\Leftarrow)}}] #1\end{itemize}}


==> include/asp-macros/semantics.tex <==
\newcommand{\true}{\ensuremath{\boldsymbol{T}}}
\newcommand{\false}{\ensuremath{\boldsymbol{F}}}

\newcommand{\Cn}[1]{\ensuremath{\mathit{Cn}(#1)}}
\newcommand{\reduct}[2]{\ensuremath{#1^{#2}}}

\newcommand{\Loops}[1]{\ensuremath{\mathit{Loop}(#1)}}

% - formulas ---------------------------------------------------------------------

\newcommand{\BF}[1]{\ensuremath{\mathit{BF}(#1)}}
\newcommand{\CF}[1]{\ensuremath{\mathit{CF}(#1)}}
\newcommand{\LF}[1]{\ensuremath{\mathit{LF}(#1)}}

\newcommand{\CFIF}[1]{\ensuremath{\overleftarrow{\mathit{CF}}(#1)}}
\newcommand{\CFFI}[1]{\ensuremath{\overrightarrow{\mathit{CF}}(#1)}}
\newcommand{\CFX}[1]{\ensuremath{\mathit{CF}^x(#1)}}

\newcommand{\ES}[2]{\ensuremath{\mathit{ES}_{\!#2}(#1)}}
\newcommand{\EB}[2]{\ensuremath{\mathit{EB}_{\!#2}(#1)}}
\newcommand{\LFS}[2]{\ensuremath{\mathit{LF}_{\!#2}(#1)}}


==> include/asp-macros/tableau.tex <==

\newcommand{\Tsigned}[1]{\ensuremath{\true{#1}}}\message{ *** RENAME, Tlit,Flit ?? *** }
\newcommand{\Fsigned}[1]{\ensuremath{\false{#1}}}

\newcommand{\TOP}[1]{\ensuremath{D_{#1}}}
\newcommand{\COP}[1]{\ensuremath{D^*_{#1}}}

\newcommand{\Proviso}[1]{\raisebox{-7pt}[0pt][0pt]{\ensuremath{(#1)}}}

\newcommand{\plit}[1]{\ensuremath{\boldsymbol{t}{#1}}}
\newcommand{\nlit}[1]{\ensuremath{\boldsymbol{f}{#1}}}


==> proofs/translation-pp2pc-proof.tex <==
\section{Proof of Theorem~\ref{thm:ppp2pcp}}


To prove Theorem~\ref{thm:ppp2pcp}, we first translate $P$  using the alternative definition $\eta^*(\mu)$ for each
subformula $\mu \in \mathit{subf}(P)$. Each definition $\eta^*(\mu)$ is then transformed into $\eta^{**}(\mu)$ by
replacing double implications by simple implications, using Lemma~\ref{lem:completion:tmp}.
Finally, $\eta^{**}(\mu)$ can be transformed into $\eta(\mu)$ as $\alwaysF\varphi$ is equivalent to
$\wnext\alwaysF\varphi \wedge \varphi$. Table~\ref{tab:ppp2tlp} shows the definitions $\eta^*$ and $\eta^{**}$.


\input{tables/table-ppp2tlp}

For practical reason, the proof uses the alternative three-valued characterization of \THT\ presented in ???.
\comment{F: add ref telf long}
Given an \HT-trace $\M$,  its associated truth valuation  is defined as a function $\trival{k}{\varphi}$ that assigns
a truth value in $\{0,1,2\}$ to formula $\varphi$ at time point $\rangeo{k}{0}{\lambda}$,  according to the
following rules:
\begin{eqnarray*}
\trival{k}{\bot} & \eqdef & 0 \\
\trival{k}{a} & \eqdef &
    \begin{cases}
    0 & \text{if} \ a \not\in T_k \\
    1 & \text{if} \ a \in T_k\setminus H_k \\
    2 & \text{if} \ a \in H_k
    \end{cases}\hspace{20pt} \text{for any atom } a\\
\trival{k}{\neg \varphi} & \eqdef &
    \begin{cases}
    2  & \text{if } \trival{k}{\varphi}=0 \\
    0  & \text{otherwise}
    \end{cases}\\
\trival{k}{\varphi \wedge \psi} & \eqdef &
    \min(\trival{k}{\varphi},\trival{k}{\psi})\\
\trival{k}{\varphi \vee   \psi} & \eqdef &
    \max(\trival{k}{\varphi},\trival{k}{\psi})\\
\trival{k}{\previous \varphi} & \eqdef &
    \begin{cases}
    0                      & \text{if } k=0 \\
    \trival{k-1}{\varphi}  & \text{if } k>0
    \end{cases}\\
\trival{k}{\varphi \since \psi} & \eqdef &
    \max\{\min(\trival{j}{\psi},\min\{\trival{i}{\varphi}\mid j<i\leq k\} ) \mid 0\leq j\leq k\}\\
\trival{k}{\varphi \trigger \psi} & \eqdef &
    \min\{\max(\trival{j}{\psi},\max\{\trival{i}{\varphi}\mid j<i\leq k\} ) \mid 0\leq j\leq k\}\\
\end{eqnarray*}

\begin{proposition}
    Let $\tuple{\H,\T}$ be an \HT-trace of length $\lambda$, ${\bm m}$ its associated valuation
    and $\rangeo{k}{0}{\lambda}$:
        \begin{itemize}
            \item $\tuple{\H,\T},k \models \varphi$ iff $\trival{k}{\varphi}=2$
            \item $\tuple{\T,\T},k \models \varphi$ iff $\trival{k}{\varphi}\neq 0$
        \end{itemize}
\end{proposition}

\vspace{1cm}

\begin{lemma}\label{lem:aux}
    Let $\varphi$ be a temporal formula over alphabet \A\ and $\tuple{\H,\T}$ an \HT-trace of length $\lambda$ over \A,
    and let $\X$ and $\Y$ be two traces of same length $\lambda$ such that $ \X\leq \Y$, $X_i\cap\A=\emptyset$ and
    $Y_i\cap\A=\emptyset$ for all $\rangeo{i}{0}{\lambda}$.
    Then, $\tuple{\H,\T}\models \varphi$ iff $\tuple{\H\cup \X,\T\cup \Y}\models \varphi$.
\end{lemma}

\begin{proofof}{Lemma~\ref{lem:aux}}
    By induction on the structure of $\varphi$.\\
\end{proofof}



We define the translation $\sigma^*$ as the present-centered program:
\begin{align*}
    \sigma^*(P) = \initial{P}\cup\final{P}\cup
    \left\lbrace \wnext\alwaysF\big(\Head{r} \leftarrow\Lab{\body{r}}\big) \mid r \in \dynamic{P} \right\rbrace
	\cup \left\lbrace \eta^*(\mu)
	\mid \mu \in \mathit{subf}(P)\right\rbrace
\end{align*}

\begin{lemma}\label{lem:nf1}
    Let $\tuple{\H,\T}$ be a \THTf{} model of length $\lambda$ of a past-present program $P$ over $\mathcal{A}$.
    Then, there exists some \THTf{}-trace $\tuple{\H',\T'}$ over alphabet $\mathcal{A}^+$
    such that $\tuple{\H,\T} = \tuple{\H',\T'}|_{\mathcal{A}}$
    and $\tuple{\H',\T'} \models \sigma^*(P)$.
\end{lemma}

\begin{proofof}{Lemma~\ref{lem:nf1}}

Take the \THTf{}-trace $\tuple{\H',\T'}$ whose three valued interpretation ${\bm m}'$ satisfies:
\begin{align}
	\trivalp{k}{\Lab{\varphi}} \overset{\label{proofofNF_equalityExtAlph}}{=} \trival{k}{\varphi}
\end{align}
for any formula $\varphi$ over $\mathcal{A}$ and for all $\rangeo{k}{0}{\lambda}$.
When $\varphi$ is an atom $a \in \mathcal{A}$ then $\trivalp{k}{a} = \trivalp{k}{\Lab{a}} = \trival{k}{a}$, which
implies that both valuations coincide for atoms, and so, $\tuple{\H',\T'} |_{\mathcal{A}} = \tuple{\H,\T}$.
It remains to be shown that $\tuple{\H',\T'} \models \sigma^*(\Gamma)$, which is equivalent to
\begin{align*}
    \tuple{\H',\T'} &\models
        \initial{P}\cup\final{P}\cup
    \left\lbrace \wnext\alwaysF\big(\Head{r} \leftarrow\Lab{\body{r}}\big) \mid r \in \dynamic{P} \right\rbrace
	\cup \left\lbrace \eta^*(\mu)
	\mid \mu \in \mathit{subf}(P)\right\rbrace\\
    \Leftrightarrow \tuple{\H',\T'} &\models
        \initial{P}\text{ and }
        \tuple{\H',\T'} \models \final{P}\text{ and }\\
    \tuple{\H',\T'}& \models
          \left\lbrace \wnext\alwaysF\big(\Head{r} \leftarrow\Lab{\body{r}}\big) \mid r \in \dynamic{P} \right\rbrace
     	  \text{ and }
        \tuple{\H',\T'} \models  \left\lbrace \eta^*(\mu \mid \mu \in \mathit{subf}(P)\right\rbrace
\end{align*}

The first two satisfaction relations follow directly from Lemma~\ref{lem:aux} as we have that $\tuple{\H,\T}$ is a model
of $P$.

Proving the third part is equivalent to proving that for all  $r \in \dynamic{P}$,
$\tuple{\H',\T'}, k \models \Head{r} \leftarrow\Lab{\body{r}} $ for all $\rangeo{k}{1}{\lambda}$.
Assume that $\tuple{\H',\T'}, k \models \Lab{\body{r}} $ for some $\rangeo{k}{1}{\lambda}$ and some $r \in \dynamic{P}$.
Then,  since $\trivalp{0}{\Lab{\gamma}}=2$ iff $\trival{0}{\gamma}=2$, we have $\tuple{\H',\T'}, k \models \body{r} $.
As $\tuple{\H,\T}$ is a model of $P$, $\tuple{\H,\T}, k \models \Head{r} \leftarrow\Lab{\body{r}}$, therefore
$\tuple{\H,\T}, k \models \Head{r}$. By Lemma~\ref{lem:aux}, we also get $\tuple{\H',\T'}, k \models \Head{r}$, and then
$\tuple{\H',\T'}, k \models \Head{r} \leftarrow\Lab{\body{r}} $.
As $k$ and $r$ where chosen arbitrarily, we get that for all  $r \in \dynamic{P}$,
$\tuple{\H',\T'}, k \models \Head{r} \leftarrow\Lab{\body{r}} $ for all $\rangeo{k}{1}{\lambda}$.

For the last part, we consider the following cases depending on the structure of the subformula $\mu$:

\begin{enumerate}
     \item
        For $\mu = \neg \varphi$ we have $\eta(\mu) = \alwaysF (\Lab{\mu} \leftrightarrow \neg\Lab{\varphi} )$ and so,
        $\tuple{\H',\T'} \models \eta(\mu)$ amounts to proving
        $\trivalp{k}{\Lab{\mu}}=\trivalp{k}{\neg\Lab{\varphi}}$ for all $\rangeo{k}{0}{\lambda}$.\\
	    In this case we have
        	\begin{align*}
	        	\trivalp{k}{\Lab{\mu}} = \trival{k}{\mu}
                &= \trival{k}{\neg\varphi}\\
                &=
                \begin{cases}
                    2  & \text{if } \trival{k}{\varphi}=0 \\
                    0  & \text{otherwise}
                \end{cases}\\
                &=
                \begin{cases}
                    2  & \text{if } \trivalp{k}{\Lab\varphi}=0 \\
                    0  & \text{otherwise}
                \end{cases}\\
                &= \trivalp{k}{\neg\Lab\varphi}\\
            \end{align*}


    \item
        For $\mu = \varphi \otimes \psi$ with $\otimes \in \{\wedge, \vee\}$ we have
        $\eta(\mu) = \alwaysF (\Lab{\mu} \leftrightarrow \Lab{\varphi} \otimes \Lab{\psi})$ and so,
        $\tuple{\H',\T'} \models \eta(\mu)$ amounts to proving
        $\trivalp{k}{\Lab{\mu}}=\trivalp{k}{\Lab{\varphi} \otimes \Lab{\psi}}$ for all $\rangeo{k}{0}{\lambda}$.\\
	    In this case we have
        	\begin{align*}
	        	\trivalp{k}{\Lab{\mu}} = \trival{k}{\mu}
                &= \trival{k}{\varphi\otimes\psi}\\
                &= f^\otimes (\trival{k}{\varphi}, \trival{k}{\psi})\\
                &= f^\otimes (\trivalp{k}{\Lab{\varphi}}, \trivalp{k}{\Lab{\psi}})\\
                &= \trivalp{k}{\Lab{\varphi} \otimes \Lab{\psi} }
            \end{align*}
        where $f^\otimes$ is the three-valued mapping associated the corresponding Boolean connective
        $\otimes \in \{\wedge, \vee, \to\}$ in the \THT{} three-valued semantics.
    \item
        For $\mu = \previous \varphi$ we have two formulas in $\eta(\mu)$:
        \begin{itemize}
            \item[-]
                For the formula $\wnext \alwaysF(\Lab\mu \leftrightarrow \previous \Lab\varphi)$ note that the prefix
                $\wnext \alwaysF$ means that the double implication must be satisfied for any $\rangeo{k}{1}{\lambda}$
                and, moreover, that this is trivially true when $\lambda=1$.
                So, we have to prove $\trivalp{k}{\Lab\mu}=\trivalp{k}{\previous \Lab\varphi}$ for all
                $\rangeo{k}{0}{\lambda}$ and may assume $\lambda>1$. The proof can be obtained as follows:
        	    \begin{align*}
		            \trivalp{k}{\Lab{\mu}} = \trival{k}{\mu}
            		&= \trival{k}{\previous \varphi}\\
            		&= \trival{k-1}{\varphi}\\
            		&= \trivalp{k-1}{\Lab\varphi}\\
            		&= \trivalp{k}{\previous \Lab{\varphi} }
            	\end{align*}
            \item[-] For satisfying the formula $\neg \Lab\mu$, this is the same than requiring $\trivalp{0}{\Lab\mu}=0$
                and this follows from $\trivalp{0}{\Lab\mu}=\trival{0}{\mu}=\trival{0}{\previous \varphi}=0$.
        \end{itemize}

    \item
        For $\mu = \varphi \since \psi$, we have to prove that
        $\trivalp{k}{\Lab{\mu}}=\trivalp{k}{\Lab{\psi} \vee ( \Lab{\varphi} \wedge \previous \Lab{\mu})}$
        for all $\rangeo{k}{0}{\lambda}$.
        This can be proved as follows:
        \begin{itemize}
            \item[--] case $k=0$
                \[\begin{array}{rll}
                    & \trivalp{0}{\Lab{\mu}}= \trival{0}{\mu} \\
                    &= \trival{0}{\varphi \since \psi}\\
                    &= \trival{0}{\psi \vee \varphi \wedge \previous \underbrace{(\varphi \since \psi)}_\mu}
                    & \text{by temporal dual of } \eqref{f:induntil}\\
                    &= \max(\trival{0}{\psi},\min(\trival{0}{\varphi},0) ) \\
                    &= \max(\trivalp{0}{\Lab\psi},\min(\trivalp{0}{\Lab\varphi},\trivalp{0}{\previous\Lab\mu}) ) \\
                    &= \trivalp{0}{\Lab\psi \vee \Lab\varphi \wedge \previous \Lab\mu}
                \end{array}\]
            \item[--] case $k>0$
                \[\begin{array}{rll}
                    & \trivalp{k}{\Lab{\mu}}= \trival{k}{\mu} \\
                    &= \trival{k}{\varphi \since \psi}\\
                    &= \trival{k}{\psi \vee \varphi \wedge \previous \underbrace{(\varphi \since \psi)}_\mu}
                    & \text{by temporal dual of } \eqref{f:induntil}\\
                    &= \max(\trival{k}{\psi},\min(\trival{k}{\varphi},\trival{k-1}{\mu}) ) \\
                    &= \max(\trivalp{k}{\Lab\psi},\min(\trivalp{k}{\Lab\varphi},\trivalp{k-1}{\Lab\mu}) ) \\
                    &= \trivalp{k}{\Lab\psi \vee \Lab\varphi \wedge \previous \Lab\mu}
                \end{array}\]
        \end{itemize}

    \item
        For $\mu = \varphi \trigger \psi$, the proof is analogous as for $\since$, exchanging the roles of $\wedge/\min$
        and $\vee/\max$ and using the temporal dual of \eqref{f:indrelease} instead of the one for \eqref{f:induntil}.
\end{enumerate}
\end{proofof}

\begin{lemma}\label{lem:nf2}
Let $\Gamma$ be a temporal theory over $\mathcal{A}$ and
let $\tuple{\H,\T}$ be a \THTf{} model of $\sigma(\Gamma)$, being ${\bm m}$ its associated three-valuation.
Then for any $\mu \in \mathit{subf}(\Gamma)$ and any $k=0..n$
we have $\trival{k}{\Lab{\mu}} = \trival{k}{\mu}$.
\end{lemma}
\begin{proofof}{Lemma~\ref{lem:nf2}}
We proceed by structural induction on $\mu$.
\begin{enumerate}
\item If $\mu$ is $\bot$ or an atom $p$, this is trivial because $\Lab\mu=\mu$ by definition.

\item If $\mu=\varphi \otimes \psi$ for any Boolean connective $\otimes \in \{\vee,\wedge,\to\}$ then:
\[\begin{array}{rll}
\trival{k}{\Lab\mu} &= \trival{k}{\Lab\varphi \otimes \Lab\psi}
& \text{using the equality in }\eta(\mu) \\
&= f^\otimes(\trival{k}{\Lab\varphi},\trival{k}{\Lab\psi}) \\
&= f^\otimes(\trival{k}{\varphi},\trival{k}{\psi})
& \text{By induction on } \varphi, \psi \\
&= \trival{k}{\varphi \otimes \psi} \\
&= \trival{k}{\mu}
\end{array}\]

\item If $\mu=\previous \varphi$ we divide into two cases:
\begin{itemize}
\item[-] If $k>0$ we can apply the first formula in $\eta(\mu)$ as follows:
\[\begin{array}{rll}
\trival{k}{\Lab\mu} &= \trival{k}{\previous \Lab\varphi}\\
&= \trival{k-1}{\Lab\varphi} & \text{(since }k>0)\\
&= \trival{k-1}{\varphi}
& \text{By induction on } \varphi \\
&= \trival{k}{\previous \varphi} \\
&= \trival{k}{\mu}
\end{array}\]
\item[-] If $k=0$ we directly use the second formula in $\eta(\mu)$ so that
    $\trival{0}{\Lab\mu}=0=\trival{0}{\previous \varphi}=\trival{0}{\mu}$.
\end{itemize}

\item If $\mu=\varphi \since \psi$ we divide into two cases:
\begin{itemize}
\item[-] If $k=0$ we directly use the second formula in $\eta(\mu)$ so that
\[\begin{array}{rll}
\trival{0}{\Lab\mu} &= \trival{0}{\Lab\psi} & \text{Using }\eta(\mu)\\
&= \trival{0}{\psi}
& \text{By induction on } \psi \\
&= \trival{0}{\varphi \since \psi}
\end{array}\]
being the last step already proved in the second case for $\since$ of Lemma~\ref{lem:nf1}.
\item[-] If $k>0$ we will proceed by a second induction on $k$.
The case $k=0$ was proved in the previous step.
So, assume it is proved up to $k-1$.
\[\begin{array}{rll}
& \trival{k}{\Lab\mu} \\
&= \trival{k}{\Lab\psi \vee (\Lab\varphi \wedge \previous \Lab\mu))}\\
&=  \max(\trival{k}{\Lab\psi}, \min(\trival{k}{\Lab\varphi},\trival{k-1}{\Lab\mu})))) \\
&=  \max(\trival{k}{\psi}, \min(\trival{k}{\varphi},\trival{k-1}{\mu}))))
& \text{Structural induction } \varphi, \psi\\
& & \text{and } k-1 \ \text{induct. on } \mu \\
&=  \trival{k}{\psi \vee \varphi \wedge \previous \mu}\\
&=  \trival{k}{\varphi \since \psi}
& \text{Temporal dual of } \eqref{f:induntil}\\
\end{array}\]
\end{itemize}

\item The case for $\mu=\varphi \trigger \psi$ is completely analogous to $\mu=\varphi \since \psi$ exchanging the roles of $\wedge/\min$ and $\vee/\max$ and using the temporal dual of \eqref{f:indrelease}.

\item If $\mu=\next \varphi$ we divide the proof into two cases:
\begin{itemize}
\item[-] If $k=n$ we use the second formula in $\eta(\mu)$ so that $\trival{n}{\Lab\mu}=0=\trival{n}{\next \varphi}=\trival{n}{\mu}$.
\item[-] If $0\leq k <n$ we can apply the first formula in $\eta(\mu)$ that guarantees $\trival{j}{\previous \Lab\mu}=\trival{j}{\Lab\varphi}$ for all $j=1..n$.
In particular, we can take $j=k+1$ and so:
\[\begin{array}{rll}
\trival{k+1}{\previous \Lab\mu} &= \trival{k+1}{\Lab\varphi}\\
&= \trival{k+1}{\varphi}
& \text{By induction on } \varphi \\
&= \trival{k}{\next \varphi} \\
&= \trival{k}{\mu}
\end{array}\]
Finally, note that $\trival{k+1}{\previous \Lab\mu}=\trival{k}{\Lab\mu}$.
\end{itemize}

\item If $\mu=\varphi \until \psi$ we have, again, two cases:
\begin{itemize}
\item[-] If $k=n$ we apply the second formula in $\eta(\mu)$ as follows
\[\begin{array}{rll}
\trival{n}{\Lab\mu} &= \trival{n}{\Lab\psi} & \text{Using }\eta(\mu)\\
&= \trival{n}{\psi}
& \text{By induction on } \psi \\
&= \trival{n}{\varphi \until \psi}
\end{array}\]
being the last step already proved in the second case for $\until$ of Lemma~\ref{lem:nf1}.


\item[-] If $0\leq k <n$ we will apply induction on $k$ backwards, from $n$ to $0$.
The case $k=n$ has been already proved.
Assume it holds for $k+1$ and we want to prove the result for $k$.
Now, the first formula in $\eta(\mu)$ that guarantees $\trival{j}{\previous \Lab\mu}=\trival{j}{\previous \Lab\psi \vee (\previous \Lab\varphi \wedge \Lab\mu)}$ for all $j=1..n$.
If we take $j=k+1$:
\[\begin{array}{rll}
\trival{k+1}{\previous \Lab\mu} &= \trival{k+1}{\previous \Lab\psi \vee (\previous \Lab\varphi \wedge \Lab\mu)}\\
&= \max(\trival{k}{\Lab\psi}),\min(\trival{k}{\Lab\varphi},\trival{k+1}{\Lab\mu}))
\end{array}\]
we can apply structural induction on subformulas $\psi$ and $\varphi$, but also integer induction on $\mu$ for case $k+1$, so we obtain that the above expression is equal to:
\[\begin{array}{rll}
&= \max(\trival{k}{\psi}),\min(\trival{k}{\varphi},\trival{k+1}{\mu})) \\
&= \trival{k}{\psi \vee \varphi \wedge \next \mu}\\
&= \trival{k}{\varphi \until \psi}
& \text{By }\eqref{f:induntil}
\end{array}\]
and, again, we have that the first line of the equations $\trival{k+1}{\previous \Lab\mu}=\trival{k}{\Lab\mu}$.
\end{itemize}

\item The case for $\mu=\varphi \release \psi$ is completely analogous to $\mu=\varphi \until \psi$ exchanging the roles of $\wedge/\min$ and $\vee/\max$ and using  \eqref{f:indrelease}.

\end{enumerate}
\end{proofof}

\begin{theorem}\label{th:thtmodels}
For any temporal theory $\Gamma$ over $\mathcal{A}$ we have that \THTf{} satisfies:
\begin{align*}
\left\lbrace  \tuple{\H,\T} \mid \tuple{\H,\T} \models \Gamma \right\rbrace =
\left\lbrace  \tuple{\H',\T'}|_\mathcal{A} \mid \tuple{\H',\T'} \models \sigma(\Gamma) \right\rbrace
\end{align*}
\end{theorem}
\begin{proofof}{th:thtmodels}
The `$\subseteq$' direction follows from Lemma~\ref{lem:nf1}.
For the `$\supseteq$' direction, take some $\tuple{\H',\T'}$ model of $\sigma(\Gamma)$ of length $n$.
This implies that its associated 3-valuation satisfies $\trivalp{0}{\Lab\varphi}=2$ for all formulas $\varphi \in \Gamma$, as those labels are included in $\sigma(\Gamma)$ as formulas.
Since $\Gamma \subseteq subf(\Gamma)$, we can apply Lemma~\ref{lem:nf2} to conclude $\trivalp{k}{\Lab\varphi}=\trivalp{k}{\varphi}$ for all $k=0..n$ but then, in particular, $2=\trivalp{0}{\Lab\varphi}=\trivalp{0}{\varphi}$ and so, $\tuple{\H',\T'}$ is also a model of $\Gamma$.
Finally, $\tuple{\H',\T'}|_\mathcal{A}$ is still a model of $\Gamma$ because the latter is a theory for vocabulary $\mathcal{A}$.
\end{proofof}

Let $\mathit{TSM}(\Gamma)$ denote the set of temporal stable models of a theory $\Gamma$.
Then:
\begin{corollary}
Let $\Gamma$ be a theory for vocabulary $\mathcal{A}$.
Then, for any theory $\Gamma'$ of the same vocabulary, \THTf{} satisfies:
\[
\mathit{TSM}(\Gamma \cup \Gamma') = \{\tuple{\H',\T'}|_\mathcal{A} \mid \tuple{\H',\T'} \in \mathit{TSM}(\sigma(\Gamma) \cup \Gamma')\}
\]
\qed
\end{corollary}

In other words, $\Gamma$ and $\sigma(\Gamma)$ are strongly equivalent, assuming we disregard the auxiliary atoms not in $\mathcal{A}$ and we use any arbitrary context $\Gamma'$ not referring to those auxiliary atoms.
%We have that \Tra{\gamma} is either of form
%\(
%\hat{\next} \alwaysF\previous \varphi \wedge \alwaysF( \finally \to \varphi)
%\)
%or
%\(
%\hat{\next} \alwaysF \varphi \wedge \alwaysF(\initially \to \varphi)
%\)
%\tbrw
%
%which means that any dynamical rule can be represented in a set of rules of the form
%\begin{align*}
%  \hat{\next} \alwaysF \alpha
%\end{align*}
%or in the form
%\begin{align*}
%  \alwaysF (\finally \to \beta),
%\end{align*}
%whereby both $\alpha$ and $\beta$ consist of literals, the unary operator $\previous$,
%the constants $\top, \bot, \initially$ and $\finally$
%and the binary operators $\wedge, \vee$ and $\to$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

